Systematic optimization of resonance parameters in a transport approach

This study optimizes resonance parameters responsible for strangeness production in the SMASH (Simulating Many Accelerated Strongly-interacting Hadrons) transport model using a genetic algorithm. By fitting resonance parameters to experimental data on exclusive strangeness cross-sections at low energies, we significantly improve the model's accuracy, especially in pion-proton interactions. Our approach explores how machine learning tools can be used for precise resonance tuning in transport approaches.

==> tables/particle_ref.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{lcccccr}
\toprule
\thead{Resonance} & \thead{Mass[GeV]} & \thead{Width[GeV]} & \thead{Mass\\Bounds[GeV]} & \thead{Width\\Bounds[GeV]} \\
\midrule
N(1440) & 1.440 & 0.350 & 0.18-0.205 & 0.18-0.205 \\
N(1520) & 1.515 & 0.110 & 0.105-0.12 & 0.105-0.12 \\
N(1535) & 1.530 & 0.150 & 0.08-0.13 & 0.08-0.13 \\
N(1650) & 1.650 & 0.125 & 0.1-0.17 & 0.1-0.17 \\
N(1675) & 1.675 & 0.145 & 0.12-0.15 & 0.12-0.15 \\
N(1680) & 1.685 & 0.120 & 0.11-0.135 & 0.11-0.135 \\
N(1700) & 1.720 & 0.200 & 0.1-0.3 & 0.1-0.3 \\
N(1710) & 1.710 & 0.140 & 0.08-0.16 & 0.08-0.16 \\
N(1720) & 1.720 & 0.250 & 0.15-0.3 & 0.15-0.3 \\
N(1875) & 1.875 & 0.250 & 0.1-0.22 & 0.1-0.22 \\
N(1880) & 1.880 & 0.400 & 0.18-0.28 & 0.18-0.28 \\
N(1895) & 1.895 & 0.120 & 0.08-0.14 & 0.08-0.14 \\
N(1900) & 1.900 & 0.200 & 0.09-0.16 & 0.09-0.16 \\
N(1990) & 1.990 & 0.500 & 0.2-0.4 & 0.2-0.4 \\
N(2060) & 2.100 & 0.400 & 0.35-0.43 & 0.35-0.43 \\
N(2080) & 2.000 & 0.350 & 0.12-0.25 & 0.12-0.25 \\
N(2100) & 2.100 & 0.260 & 0.24-0.34 & 0.24-0.34 \\
N(2120) & 2.120 & 0.300 & 0.2-0.36 & 0.2-0.36 \\
N(2190) & 2.180 & 0.400 & 0.3-0.5 & 0.3-0.5 \\
N(2220) & 2.220 & 0.400 & 0.36-0.48 & 0.36-0.48 \\
N(2250) & 2.250 & 0.470 & 0.35-0.5 & 0.35-0.5 \\
$\Delta$(1620) & 1.610 & 0.130 & 0.08-0.14 & 0.08-0.14 \\
$\Delta$(1700) & 1.710 & 0.300 & 0.2-0.3 & 0.2-0.3 \\
$\Delta$(1900) & 1.860 & 0.250 & 0.18-0.3 & 0.18-0.3 \\
$\Delta$(1905) & 1.880 & 0.330 & 0.26-0.34 & 0.26-0.34 \\
$\Delta$(1910) & 1.900 & 0.300 & 0.2-0.5 & 0.2-0.5 \\
$\Delta$(1920) & 1.920 & 0.300 & 0.2-0.4 & 0.2-0.4 \\
$\Delta$(1930) & 1.950 & 0.300 & 0.3-0.45 & 0.3-0.45 \\
$\Delta$(1950) & 1.930 & 0.280 & 0.22-0.26 & 0.22-0.26 \\
\bottomrule
\end{tabular}
\caption{Tabulation of the default resonance masses and widths in SMASH-3.1 and bounds used.}
\label{tab:part-ref}
\end{table}
